Manekko: Training Small but Foundational 3D Medical Models by Mimicking Natural Vision Model Features

Self-supervised learning (SSL) for 3D medical imaging typically learns representations directly from unlabelled volumes. We study whether features from pretrained 2D natural-image models provide effective targets to train 3D medical vision foundation models. Our method, Manekko, extracts features from axial, coronal, and sagittal slices, normalizes them using foreground statistics, and trains a 3D encoder to regress to the resulting patch and affinity statistics. We pretrain separate models on brain MRI and multi-anatomy CT and evaluate over various anatomies, modalities and tasks. Across 15 segmentation datasets, Manekko achieves matches or exceeds in mean DSC among the evaluated encoders, both frozen and after full fine-tuning, with approximately 8x fewer encoder parameters and 18x fewer medical pretraining volumes compared to larger encoders. Additional frozen classification, regression, and retrieval evaluations demonstrate the utility of Manekko's global representations. We find that across seven reference models to regress from, in-context scene understanding on natural images strongly correlates with frozen segmentation evaluation providing a recipe to choose a reference model pre-hoc. These results support natural-image features as effective targets for training 3D medical foundation models.

==> tables/supp_memory.tex <==
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l c cc}
    \toprule
    & \textbf{Params (M)} & \multicolumn{2}{c}{\textbf{Memory (GiB)}} \\
    \cmidrule(lr){2-2}\cmidrule(lr){3-4}
    Encoder & Enc.\ + Dec. & Peak & Fwd.\ extra \\
    \midrule
    \rowcolor{oursrow}
    \ours                             & 74.9  & 4.17 & 4.05 \\
    Primus-M                          & 163.0 & 4.72 & 4.12 \\
    3DINO~\cite{3dino}                & 334.9 & 5.28 & 4.02 \\
    nnFoundation~\cite{nnfoundation}  & 558.5 & 6.29 & 4.15 \\
    \bottomrule
\end{tabular}

